Photon Statistics of Filtered Resonance Fluorescence

Spectral filtering of resonance fluorescence is widely employed to improve single photon purity and indistinguishability by removing unwanted backgrounds. For filter bandwidths approaching the emitter linewidth, complex behaviour is predicted due to preferential transmission of components with differing photon statistics. We probe this regime using a Purcell-enhanced quantum dot in both weak and strong excitation limits, finding excellent agreement with an extended sensor theory model. By changing only the filter width, the photon statistics can be transformed between antibunched, bunched, or Poissonian. Our results verify that strong antibunching and a sub-natural linewidth cannot simultaneously be observed, providing new insight into the nature of coherent scattering.

==> xx.tex <==


